Dimers and M-Curves: Limit Shapes from Riemann Surfaces

We present a general approach for the study of dimer model limit shape problems via variational and integrable systems techniques. In particular we deduce the limit shape of the Aztec diamond and the hexagon for quasi-periodic weights through purely variational techniques. Putting an M-curve at the center of the construction allows one to define weights and algebro-geometric structures describing the behavior of the corresponding dimer model. We extend the quasi-periodic setup of our previous paper [7] to include a diffeomorphism from the spectral data to the liquid region of the dimer. Our novel method of proof is purely variational and exploits a duality between the dimer height function and its dual magnetic tension minimizer and applies to dimers with gas regions. We apply this to the Aztec diamond and hexagon domains to obtain explicit expressions for the complex structure of the liquid region of the dimer as well as the height function and its dual. We compute the weights and the limit shapes numerically using the Schottky uniformization technique. Simulations and predicted results match completely.

==> Sections/08_Cardioid.tex <==
\section{Cardioid Case}
\label{sec:08_cardioid}

\NOTE{
	\begin{itemize}
		\item $\hat{\mathcal{R}}$ quadruple cover of $\mathcal{R}$
		\item Again count zeros. Defines liquid map $\Omega$.
		\item $\Omega: \mathcal{F}_R \to \hat{\mathcal{R}}_+^\circ$ diffeomorphism.
		\item Parameter $r$ from triple zero at $0$.
		\item Calculate touching points. $\implies$ consistent with boundary conditions.
		\item reflection symmetric liquid region.
		\item All other arguments (Burgers, tangentiality, extension, tangent zeros, local convexity) same as Aztec diamond $\implies$ minimality.
		\item Picture
	\end{itemize}
}

==> Sections/09_GeneralCase.tex <==
\section{General Case}
\label{sec:09_general_case}

\NOTE{
    \begin{itemize}
        \item Fixed $\calR, \{\alpha, \beta\}, d\zeta_1, d\zeta_2$.
        \item Covering $\hat{\calR}$ with $d\zeta_3$ on it with singularities in points projecting to $\{\alpha, \beta\}$. 
        \item If this gives a bijection from $\hat{\calR}$ to liquid zone, can construct boundary conditions around that liquid region.
        \item Call such boundary conditions integrable?
    \end{itemize}
}

==> Sections/11_Computation.tex <==
\section{Computation}
\label{sec:11_Computation}

One of the benefits of working with Schottky groups is that we get expressions for the Fock weights $K_{wb}$, the differentials $d\zeta_k$ and their integrals $\zeta_k$ in terms of (converging) Poincaré series. This setup makes it practical to numerically compute all those values. 

We utilize this approach to obtain samples of dimer configurations weights coming from some given Harnack data $\cubr{\mathcal{S}, \mathcal{T}}$ overlaid with predicted arctic curves on both the Aztec diamond and the hexagon. 

We utilize the jtem library introduced in \cite{schmies_computational_2005} for computations of theta functions and summations over Schottky groups. The face weights \eqref{eq:Fock_face_weight} that the graph is populated with are computed using Theorem~\ref{thm:Schottky_series} for the $B$ matrix. For approximation methods of theta functions see \cite{schmies_computational_2005}. We use a simple Metropolis-Hastings sampling algorithm with those weights that we have implemented on the GPU for more efficient sampling, see \cite{keating_random_2018,BBS}. This yields only approximate sampling. In the examples of the Aztec diamond and hexagon there are shuffling algorithms available that obtain efficient exact sampling, see \cite{Gorin_2021} for an overview. We have chosen not to use those as we hope to be able extend our methods to other setups and regions.

Proposition~\ref{prop:zeta_Schottky} allows for computation of $d\zeta_k$ as well as $\zeta_k$. Evaluating \eqref{eq:xy_on_real_ovals} on the real ovals then yields the predicted arctic curves. We see that the predictions and sampled configurations match well, see e.g. Figures~\ref{fig:main_aztec_config}, \ref{fig:main_hex_config}.

For the hexagon in the ramified case we impose the condition that the Harnack data $\hat{\mathcal{S}}$ must define an admissible $d\zeta_3 = f(z) dz$ i.e. $f_3(0) = 0$, see Definition~\ref{def:hex_Harnack_data_admissible_ramified}. This is generically not true so starting with just any symmetric $\hat{\mathcal{S}}$ does not satisfy this. In order to find an admissible $\hat{S}$ we run an optimization on the train track parameters $\cubr{\alpha^\pm_i, \beta^\pm_j, \gamma^\pm_l}$ utilizing derivatives of $f_3$ at the point $0$ with respect to the train track parameters. This does not change the Riemann surface and typically only moves the train track parameters a little bit to obtain admissible data. Since the train track angles do not move much this approach yields good control of the final picture when chosing the initial parameters $\hat{\mathcal{S}}$.

% \TODO{Remark or maybe subsection about more efficient computation under existence of symmetry $\pi$ for hexagon?}


